People on Drugs: Credibility of User Statements in Health Communities

Online health communities are a valuable source of information for patients and physicians. However, such user-generated resources are often plagued by inaccuracies and misinformation. In this work we propose a method for automatically establishing the credibility of user-generated medical statements and the trustworthiness of their authors by exploiting linguistic cues and distant supervision from expert sources. To this end we introduce a probabilistic graphical model that jointly learns user trustworthiness, statement credibility, and language objectivity. We apply this methodology to the task of extracting rare or unknown side-effects of medical drugs --- this being one of the problems where large scale non-expert data has the potential to complement expert medical knowledge. We show that our method can reliably extract side-effects and filter out false statements, while identifying trustworthy users that are likely to contribute valuable medical information.

==> log <==
Index: kdd14.tex
===================================================================
--- kdd14.tex	(revision 110)
+++ kdd14.tex	(revision 117)
@@ -21,24 +21,36 @@
 
 \begin{document}
 
+
+\numberofauthors{1} %  in this sample file, there are a *total*
+% of EIGHT authors. SIX appear on the 'first-page' (for formatting
+% reasons) and the remaining two appear in the \additionalauthors section.
+%
+\newcommand{\authspace}{\hspace*{.2in}}
+\author{
+Subhabrata Mukherjee$^*$ \authspace  Gerhard Weikum$^*$  \authspace \mbox{Cristian Danescu-Niculescu-Mizil$^\dagger$}\\
+ \affaddr{$^*$Max Planck Institute for Informatics, $^\dagger$Max Planck Institute for Software Systems} \\
+ \email{smukherjee@mpi-inf.mpg.de, weikum@mpi-inf.mpg.de}, cristian@mpi-sws.org}
+
+
 \title{People on Drugs: \\ Credibility of User Statements in Health Communities}
 
 
-\numberofauthors{3}
-\author{
-\alignauthor Subhabrata Mukherjee \\
-\affaddr{Max Planck Institute for Informatics} \\
-\affaddr{Saarbr\"ucken, Germany} \\
-\email{smukherjee@mpi-inf.mpg.de}
-\alignauthor Gerhard Weikum \\
-\affaddr{Max Planck Institute for Informatics} \\
-\affaddr{Saarbr\"ucken, Germany} \\
-\email{weikum@mpi-inf.mpg.de}
-\alignauthor Cristian Danescu-Niculescu-Mizil \\
-\affaddr{Max Planck Institute for Software Systems} \\
-\affaddr{Saarbr\"ucken, Germany} \\
-\email{cristian@mpi-sws.org}
-}
+% \numberofauthors{3}
+% \author{
+% \alignauthor Subhabrata Mukherjee \\
+% \affaddr{Max Planck Institute for Informatics} \\
+% \affaddr{Saarbr\"ucken, Germany} \\
+% \email{ smukherjee@mpi-inf.mpg.de}
+% \alignauthor Gerhard Weikum \\
+% \affaddr{Max Planck Institute for Informatics} \\
+% \affaddr{Saarbr\"ucken, Germany} \\
+% \email{  weikum@mpi-inf.mpg.de}
+% \alignauthor Cristian Danescu-Niculescu-Mizil \\
+% \affaddr{Max Planck Institute for Software Systems} \\
+% \affaddr{Saarbr\"ucken, Germany} \\
+% \email{  cristian@mpi-sws.org}
+% }
 
 
 \newcommand{\squishlist}{


==> tmp <==
% !TEX root = kdd14.tex

\section{Introduction}


%social media in general and health forums in particular
Online social media includes a wealth of topic-specific communities and discussion forums about politics, music, health, and many other domains. User-generated content in such communities offer a great potential for distilling and analyzing facts and opinions.   
In particular, online health communities constitute an important source of information for patients and doctors alike, 
with 59\% of the adult U.~S. population consulting online health resources \cite{Fox:PewInternetAndAmericanLifeProject:2013},
and nearly half of U.~S. physicians relying on online resources \cite{IMS2014} for professional use.  

One of the major hurdles preventing the full exploitation of information from online health communities is the widespread concern regarding the quality and credibility of user-generated content \cite{Peterson:JMedInternetRes:2003,cline2001consumer,white2014health}. To address this issue, this work proposes a system that can automatically assess the credibility of medical statements made by users of online health communities.
In particular, we focus on extracting rare or unknown side-effects effects of drugs --- this being one of the problems where large scale non-expert data has the potential to complement expert medical knowledge \cite{White2014}, but where misinformation can have life-threatening consequences.

\comment{
Patients engage in discussions with other patients and doctors about their experience with medical drugs and therapies, including negative side-effects of drugs or drug combinations. In contrast to the conversative statements in official sources like {\small\tt \href{http://www.fda.gov}{fda.gov}} or {\small\tt \href{http://www.ema.europa.eu/ema/}{ema.europa.eu}}, such communities provide insight on which side-effects are {\em actually observed} and 
under
which specific conditions.
}

% As a point in case, consider health forums such as {\small\tt \href{http://www.healthboards.com/}{healthboards.com}} or {\small\tt \href{http://www.patient.co.uk/}{patient.co.uk}}, as the focus of this paper. Here, patients engage in discussions with other patients and doctors about their experience with medical drugs and therapies, including negative side-effects of drugs or drug combinations. In contrast to the conversative statements in official sources like {\small\tt \href{http://www.fda.gov}{fda.gov}} or {\small\tt \href{http://www.ema.europa.eu/ema/}{ema.europa.eu}}, such communities provide insight on which side-effects are {\em actually observed} and 
% under
% which specific conditions.
% %GW: the next sentence does not add anything, hence commented out
% \comment{
% The posts contributed by actual users of the drugs can provide large-scale information on the drug-habits of 
% users, drug usage and interactions,  and can even provide insight into the unreported side-effects of drugs.
% }%\comment
% According to an empirical study xx, even many medical doctors regularly consult online sources such as Wikipedia and specialized health forums. 

%problem of uncertainty
We can apply information extraction (IE) methods using probabilistic graphical models \cite{Sarawagi2008,KollerFriedman2009} to user posts in online forums, thus obtaining statements in the form of subject-predicate-object (SPO) triples like {\em $<$drug$>$ hasSideEffect $<$symptom$>$}. We use a tool developed by~\cite{Ernst2014} to identify side-effects in statements. However, social media often exhibit a lot of noise, bias, subjectivity, and distorted if not plainly false statements. Thus, even for health-centric communities, the output of IE methods has inherent uncertainty. Our goal in this paper is to infer the {\em credibility} of SPO statements.

%factors: subjectivity of language, trustworthiness of users, credibility of statements
We can harness three factors to assess the credibility of a statement $s$ extracted from a post $p$ of user $u$:
\squishlist
\item {\em Users:} the overall {\em trustworthiness} (or authority or reputation) of user $u$, as expressed by her status and engagement in the community.
%subho:camera-ready
This is measured by the source's conformity to truth, or the proportion of true facts mentioned by the source.
% in the form of the number of \textit{questions and answers posted}, 
%interactions with other users in the form of \textit{replies, likes, etc.}, 
%and other user-specific properties like \textit{user demographics};
\item {\em Language:} the {\em objectivity}, rationality (as opposed to emotionality), and general quality of the language expressions 
%in the form of \textit{discourse} and \textit{affective emotions} 
that $u$ uses in her posts, across all topics.
%subho:camera-ready
Objectivity is the quality of the post to be free from preference, emotion, bias and prejudice of the author.
\item {\em Statements:} the {\em credibility} (or truthfulness) of the user's  statements
%across all her posts, as many good statements strengthen the credibility of a new statement $s$.
across all users' posts, as objective observations strengthen the credibility of a statement.
\squishend

%cross-talk of the three aspects
These factors have a strong influence on each other. We consider a statement more credible if it is posted by a trustworthy user and expressed in confident and objective language. Consider the following review about the drug ``Depo-Provera'' by a senior member of {\small\tt \href{http://www.healthboards.com/}{healthboards.com}}:
``{\small \dots Depo is very dangerous as a birth control and has too many long term side-effects like reducing bone density \dots}''
From this post, we can derive the SPO statement {\em Depo hasSideEffect reducedBoneDensity}. Conversely, high subjectivity and emotionality in a post suggest lower credibility of statements and lower believability in that user's contents. A negative example along these lines is: \\
%subho:camera-ready
``{\small I have been on the same cocktail of meds (10 mgs. Elavil at bedtime/60-90 mgs. of Oxycodone during the day/1/1/2 mgs. Xanax a day....once in a while I have really bad hallucination type dreams. I can actually ``feel" someone pulling me of the bed and throwing me around. I know this sounds crazy but at the time it fels somewhat demonic.}''
Although this post suggests the statement {\em Xanax hasSideEffect hallucination},
the style of the post does not give it high credibility.
%GW: we may want to pick a different example - hallucinations may be among the true side effects of Prozac

This shows that in order to identify credible SPO statements, we also need to assess the trustworthiness of users and the objectivity of the user language. Therefore, the problem that we address in this paper is the {\em joint analysis of statements, users, and language}
in social media about health topics. To the best of our knowledge, this problem has not been studied in prior work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Approach and Contribution}

%our approach in a nutshell: feature model first
Our approach first identifies a rich set of features for each of the three factors: statements, users and language. Features include user-specific properties like gender, thread-specific properties like posts, number of questions, answers, thanks, etc., 
 and document length statistics like words per post, sentences per post, etc. 
 On the language side, we perform linguistic analyses to extract {stylistic} and {affective} features from user posts. Discourse features help to identify authoritative user statements by examining the usage of modals, negation, inferential and violating conjunctions, hypothetical statements, definitives, density of nouns (names of drugs, diseases, symptoms), frequency of adjectives and adverbs etc. Affective features help to identify objective statements  by analyzing user emotions in the post like anxiety, depression, esteem, confidence, sympathy, coolness, etc.  We establish a baseline for identifying potential side-effects of drugs 
from user posts by training an SVM over this comprehensive feature model. 
%GW: the following sentence is potentially misleading, hence dropped
%Since the number of positive side-effects of a drug is typically less, 
%we use the notion of \textit{distant supervision} to create an expanded training set.

%our approach in a nutshell: now the probabilistic model
The main contribution of this paper is a probabilistic graphical model tailored to the problem setting that facilitates joint inference over users, language, and statements.
%Our model captures cross-talk between users and their statements, 
%for example, a user gaining trust by making statements that agree with highly reputed users. 
We devise a Markov Random Field (MRF) with individual users, posts, and statements as nodes.
The quality of these nodes -- trustworthiness, objectivity, and credibility --
is modeled as binary random variables.
Our method is semi-supervised with a subset of training statements, 
derived from expert databases, labeled as true or false.
We use features for users and posts
that can be directly observed in a health community.
We use an EM (Expectation-Maximization)
framework for inference and parameter estimation, where we employ MCMC sampling
%for MAP inference on our MRF model 
in the \textit{E-step} for estimating the label of unknown statements; whereas feature weights are computed by Trust Region Newton method~\cite{Lin2008}
%with L2 regularization 
in the \textit{M-step}
%subho:camera-ready
from \textit{partial expert information}.

%results: experiments, findings
We apply our method to
%$2.7$ 
$2.8$ %see experiments section
million posts by $1,500$ users of the online community {\small\tt \href{http://www.healthboards.com/}{healthboards.com}}. Our MRF model achieves an overall accuracy of $82.18\%$ in
identifying drug side-effects,
with an improvement of $13\%$ and $4\%$ over SVM baseline without and with \textit{distant supervision}, respectively.
%GW: double-check these accuracy figures and make consistent with experiments section
%
%GW: the next two sentences are risky here, as one may interpret this counting rare side effects as false - which we should not do
%GW: perhaps better drop these two sentences here
\comment{It is more difficult to identify false statements, as these are frequently reported -- often in
an affective and non-credible manner -- by 
misguided laymen.
Our graphical model outperforms the SVM baseline in identifying the negative instances.}
We believe our model can be a strong asset for possible in-depth analysis, like determining the specific conditions (age, gender, social group, life style, other medication, etc.) under which side-effects are observed.

%novel contributions
In a nutshell, the novel contributions of this paper are:
\squishlist
\item {\em Model:} We propose a model to capture the mutual influence of user trustworthiness, language objectivity, and statement credibility
in social media, and we devise a comprehensive feature model to this end.
\item {\em Method:} We develop a method for joint inference over users, language, and statements by a judiciously designed probabilistic
graphical model.
\item {\em Application:} We apply this methodology to the problem of extracting side-effects of medical drugs from online discussion forums about health.
\squishend

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent{\bf Outline:}
The rest of the paper is organized as follows.
Section~\ref{sec:model} introduces our computational model.
Section~\ref{sec:features} discusses the language and user features that we harness.
Section~\ref{sec:inference} presents the algorithms we employ for probabilistic inference.
Section~\ref{sec:experiments} gives an experimental evaluation over real-life data from {\small\tt \href{http://www.healthboards.com/}{healthboards.com}}.
Section~\ref{sec:usecases} presents two use-case studies, with the goals of discovering rare side-effects
of drugs and inferring which users one should trust and follow.
Section~\ref{sec:relatedwork} discusses related work.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%

%%C: previous version
\comment{
\section{Introduction}

\subsection{Motivation and Problem}

%social media in general and health forums in particular
Social media on the Internet is not just about Facebook and Twitter, but also includes a wealth of topic-specific online communities and discussion forums about politics, music, health, and many other domains. These user-generated contents have a great value for distilling and analyzing observations, opinions, and statements in large user communities. As a point in case, consider health forums such as {\small\tt \href{http://www.healthboards.com/}{healthboards.com}} or {\small\tt \href{http://www.patient.co.uk/}{patient.co.uk}}, as the focus of this paper. Here, patients engage in discussions with other patients and doctors about their experience with medical drugs and therapies, including negative side-effects of drugs or drug combinations. In contrast to the conversative statements in official sources like {\small\tt \href{http://www.fda.gov}{fda.gov}} or {\small\tt \href{http://www.ema.europa.eu/ema/}{ema.europa.eu}}, such communities provide insight on which side-effects are {\em actually observed} and 
under
which specific conditions.
%GW: the next sentence does not add anything, hence commented out
\comment{
The posts contributed by actual users of the drugs can provide large-scale information on the drug-habits of 
users, drug usage and interactions,  and can even provide insight into the unreported side-effects of drugs.
}%\comment
According to an empirical study \cite{IMS2014}, even many medical doctors regularly consult online sources such as Wikipedia and specialized health forums. 

%problem of uncertainty
We can apply information extraction (IE) methods using probabilistic graphical models \cite{Sarawagi2008,KollerFriedman2009} to user posts in online forums, thus obtaining statements in the form of subject-predicate-object (SPO) triples like {\em $<$drug$>$ hasSideEffect $<$symptom$>$}. We use a tool developed by~\cite{Ernst2014} to identify side-effects in statements. However, social media often exhibit a lot of noise, bias, subjectivity, and distorted if not plainly false statements. Thus, even for health-centric communities, the output of IE methods has inherent uncertainty. Our goal in this paper is to infer the {\em credibility} of SPO statements.

%factors: subjectivity of language, trustworthiness of users, credibility of statements
We can harness three factors to assess the credibility of a statement $s$ extracted from a post $p$ of user $u$:
\squishlist
\item {\em Users:} the overall {\em trustworthiness} (or authority or reputation) of user $u$, as expressed by her status and engagement in the community.
%subho:camera-ready
This is measured by the source's conformity to truth, or the proportion of true facts mentioned by the source.
% in the form of the number of \textit{questions and answers posted}, 
%interactions with other users in the form of \textit{replies, likes, etc.}, 
%and other user-specific properties like \textit{user demographics};
\item {\em Language:} the {\em objectivity}, rationality (as opposed to emotionality), and general quality of the language expressions 
%in the form of \textit{discourse} and \textit{affective emotions} 
that $u$ uses in her posts, across all topics.
%subho:camera-ready
Objectivity is the quality of the post to be free from preference, emotion, bias and prejudice of the author.
\item {\em Statements:} the {\em credibility} (or truthfulness) of the user's  statements
%across all her posts, as many good statements strengthen the credibility of a new statement $s$.
across all users' posts, as objective observations strengthen the credibility of a statement.
\squishend

%cross-talk of the three aspects
These factors have a strong influence on each other. We consider a statement more credible if it is posted by a trustworthy user and expressed in confident and objective language. Consider the following review about the drug ``Depo-Provera'' by a senior member of {\small\tt \href{http://www.healthboards.com/}{healthboards.com}}:
``{\small \dots Depo is very dangerous as a birth control and has too many long term side-effects like reducing bone density \dots}''
From this post, we can derive the SPO statement {\em Depo hasSideEffect reducedBoneDensity}. Conversely, high subjectivity and emotionality in a post suggest lower credibility of statements and lower believability in that user's contents. A negative example along these lines is: \\
%subho:camera-ready
``{\small I have been on the same cocktail of meds (10 mgs. Elavil at bedtime/60-90 mgs. of Oxycodone during the day/1/1/2 mgs. Xanax a day....once in a while I have really bad hallucination type dreams. I can actually ``feel" someone pulling me of the bed and throwing me around. I know this sounds crazy but at the time it fels somewhat demonic.}''
Although this post suggests the statement {\em Xanax hasSideEffect hallucination},
the style of the post does not give it high credibility.
%GW: we may want to pick a different example - hallucinations may be among the true side effects of Prozac

This shows that in order to identify credible SPO statements, we also need to assess the trustworthiness of users and the objectivity of the user language. Therefore, the problem that we address in this paper is the {\em joint analysis of statements, users, and language}
in social media about health topics. To the best of our knowledge, this problem has not been studied in prior work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Approach and Contribution}

%our approach in a nutshell: feature model first
Our approach first identifies a rich set of features for each of the three factors: statements, users and language. Features include user-specific properties like gender, thread-specific properties like posts, number of questions, answers, thanks, etc., 
 and document length statistics like words per post, sentences per post, etc. 
 On the language side, we perform linguistic analyses to extract {stylistic} and {affective} features from user posts. Discourse features help to identify authoritative user statements by examining the usage of modals, negation, inferential and violating conjunctions, hypothetical statements, definitives, density of nouns (names of drugs, diseases, symptoms), frequency of adjectives and adverbs etc. Affective features help to identify objective statements  by analyzing user emotions in the post like anxiety, depression, esteem, confidence, sympathy, coolness, etc.  We establish a baseline for identifying potential side-effects of drugs 
from user posts by training an SVM over this comprehensive feature model. 
%GW: the following sentence is potentially misleading, hence dropped
%Since the number of positive side-effects of a drug is typically less, 
%we use the notion of \textit{distant supervision} to create an expanded training set.

%our approach in a nutshell: now the probabilistic model
The main contribution of this paper is a probabilistic graphical model tailored to the problem setting that facilitates joint inference over users, language, and statements.
%Our model captures cross-talk between users and their statements, 
%for example, a user gaining trust by making statements that agree with highly reputed users. 
We devise a Markov Random Field (MRF) with individual users, posts, and statements as nodes.
The quality of these nodes -- trustworthiness, objectivity, and credibility --
is modeled as binary random variables.
Our method is semi-supervised with a subset of training statements, 
derived from expert databases, labeled as true or false.
We use features for users and posts
that can be directly observed in a health community.
We use an EM (Expectation-Maximization)
framework for inference and parameter estimation, where we employ MCMC sampling
%for MAP inference on our MRF model 
in the \textit{E-step} for estimating the label of unknown statements; whereas feature weights are computed by Trust Region Newton method~\cite{Lin2008}
%with L2 regularization 
in the \textit{M-step}
%subho:camera-ready
from \textit{partial expert information}.

%results: experiments, findings
We apply our method to
%$2.7$ 
$2.8$ %see experiments section
million posts by $1,500$ users of the online community {\small\tt \href{http://www.healthboards.com/}{healthboards.com}}. Our MRF model achieves an overall accuracy of $82.18\%$ in
identifying drug side-effects,
with an improvement of $13\%$ and $4\%$ over SVM baseline without and with \textit{distant supervision}, respectively.
%GW: double-check these accuracy figures and make consistent with experiments section
%
%GW: the next two sentences are risky here, as one may interpret this counting rare side effects as false - which we should not do
%GW: perhaps better drop these two sentences here
\comment{It is more difficult to identify false statements, as these are frequently reported -- often in
an affective and non-credible manner -- by 
misguided laymen.
Our graphical model outperforms the SVM baseline in identifying the negative instances.}
We believe our model can be a strong asset for possible in-depth analysis, like determining the specific conditions (age, gender, social group, life style, other medication, etc.) under which side-effects are observed.

%novel contributions
In a nutshell, the novel contributions of this paper are:
\squishlist
\item {\em Model:} We propose a model to capture the mutual influence of user trustworthiness, language objectivity, and statement credibility
in social media, and we devise a comprehensive feature model to this end.
\item {\em Method:} We develop a method for joint inference over users, language, and statements by a judiciously designed probabilistic
graphical model.
\item {\em Application:} We apply this methodology to the problem of extracting side-effects of medical drugs from online discussion forums about health.
\squishend

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent{\bf Outline:}
The rest of the paper is organized as follows.
Section~\ref{sec:model} introduces our computational model.
Section~\ref{sec:features} discusses the language and user features that we harness.
Section~\ref{sec:inference} presents the algorithms we employ for probabilistic inference.
Section~\ref{sec:experiments} gives an experimental evaluation over real-life data from {\small\tt \href{http://www.healthboards.com/}{healthboards.com}}.
Section~\ref{sec:usecases} presents two use-case studies, with the goals of discovering rare side-effects
of drugs and inferring which users one should trust and follow.
Section~\ref{sec:relatedwork} discusses related work.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}

==> veracity <==
\cd{Fix figure: TrustWorthiness -> Trustworthiness}  \cd{Throughout the paper: decapitalize captions(e.g., ``Interaction between Statements and Users''--> ``Interactions between statements and users.''; note the ending period), since thesea re actual sentences, not titles.  When in doubt, see also the style guides for sig-alternate: \url{http://www.acm.org/sigs/publications/sig-alternate.pdf}}}

